Distributionally Robust Control with Constraints on Linear Unidimensional Projections

Distributionally robust control is a well-studied framework for optimal decision making under uncertainty, with the objective of minimizing an expected cost function over control actions, assuming the most adverse probability distribution from an ambiguity set. We consider an interpretable and expressive class of ambiguity sets defined by constraints on the expected value of functions of one-dimensional linear projections of the uncertain parameters. Prior work has shown that, under conditions, problems in this class can be reformulated as finite convex problems. In this work, we propose two iterative methods that can be used to approximately solve problems of this class in the general case. The first is an approximate algorithm based on best-response dynamics. The second is an approximate method that first reformulates the problem as a semi-infinite program and then solves a relaxation. We apply our methods to portfolio construction and trajectory planning scenarios.

==> sections/prior.tex <==
\section{Background}\label{sec:priorwork}
% \subsection{Distributionally Robust Optimization}
%\textcolor{red}{[A]:Need to make sure we fix notation. Maybe no math in background.}

% Classical optimization under uncertainty often assumes a known probability distribution of the uncertainties. For example, in stochastic optimization, empirical risk minimization (ERM) optimizes an objective function $l$ that estimates costs given disturbances $x$, distributed according to a known distribution $\mathbb{P}$, and design inputs $u$: $u^*_{\text{ERM}} = \arg\min_{u\in\mathcal{U}} \mathbb{E}_{x \sim \mathbb{P}} [l(u,x)]$~\cite{boyd2009convex}. In practice, assuming a known probability distribution can be fragile -- if the true distribution deviates from the assumed model, the solution's performance can deteriorate severely.
% %The goal of optimization is to find the design inputs $x$ in a set $\mathcal{X}$ that minimize an objective function $l: \mathcal{X} \to \mathbb{R}$ that models the expected cost of following a routine parameterized by those design inputs, $\min_{x\in \mathcal{X}} l(x)$.
% %However, in many practical decision-making applications, real-world disturbances can induce changes to the routines that accrue cost. 
% Robust optimization addresses this by optimizing against the worst-case disturbance realization within a prespecified set $\mathcal{X}$, $u^*_{\text{robust}} = \arg\min_{u\in\mathcal{U}}\max_{x \in \mathcal{X}} l(x, d)$~\cite{ben2002robust,bertsimas2011theory}. Unfortunately, specifying a complete and accurate disturbance set $\mathcal{U}$ a priori can be impractical. Additionally, worst-case optimization can be overly pessimistic against the real disturbances.

Distributionally robust optimization (DRO) bridges the gap between stochastic and robust optimization by considering uncertainty in the probability distribution. Rather than assuming a known disturbance distribution or set, DRO assumes instead that the true disturbance distribution can come from a set of distributions $\mathcal{S}_\mathbb{P}$, called the ambiguity set, that is often chosen to be close to a nominal (e.g. empirical) distribution $\hat{\mathbb{P}}$. This yields a minimax problem: choose a decision to minimize the cost, assuming an adversary will choose a distribution that maximizes the cost, 
\begin{equation}
    u^*_{\text{DRO}} = \arg\min_{u\in\mathcal{U}} \max_{\mathbb{P} \in \mathcal{S}_{\mathbb{P}}}\mathbb{E}_{x \sim \mathbb{P}}[l(u, x)]\text{.} 
\end{equation}
By optimizing against the worst-case distribution, DRO provides distributional robustness without being overly pessimistic or prescriptive about disturbances~\cite{rahimian2022frameworks, lin2022distributionally}.

Solution methods typically reformulate the problem as a semi-infinite program
satisfying constraints over all members of $\mathcal{S}_\mathbb{P}$. They then dualize the problem~\cite{delage2010distributionally,wiesemann2014distributionally}, or iteratively relax the constraints into representative atomic subsets of $\mathcal{S}_\mathbb{P}$~\cite{pflug2007ambiguity,rahimian2019identifying}. 
Typical choices for ambiguity sets consider distributions within an $\epsilon$-ball around a nominal distribution $\hat{\mathbb{P}}$, $\mathcal{S}_\mathbb{P} = \{\mathbb{P} : D(\mathbb{P},\hat{\mathbb{P}}) \leq \epsilon\}$, defined by a discrepancy measure $D$, such as KL divergence~\cite{ben2013robust,hu2013kullback}, other general $f$-divergences~\cite{namkoong2016stochastic,duchi2021learning}, or Wasserstein distances~\cite{kuhn2019wasserstein, gao2024wasserstein}. 
However, efficient solutions to DRO have been considered for many uncertainty sets~\cite{rahimian2022frameworks,lin2022distributionally}. 
A common challenge across the choice of ambiguity sets, however, remains the selection and interoperability of hyperparameters (e.g. the discrepancy radius $\epsilon$), which can significantly affect both robustness and conservatism.

%\FIXME{track down projected Wasserstein DRO paper for tractability in high dims}. \FIXME{Discuss duality -- Strong duality of KL discrepancy ball\ndref and of more ambiguity sets \cite{zhen2023unified}. }

% Discuss ambiguity sets in greater detail, e.g. 

Recent works have studied the application of DRO to control, where design variables represent sequential control actions $u_{1:T}$ and disturbances arise from uncertain dynamics and observations. In continuous control settings, moment-based DRO methods enable robust chance-constrained policies~\cite{van2015distributionally}, while Wasserstein-based DRO methods provide data-driven solutions for linear-quadratic problems, applicable to fully observable~\cite{yang2020wasserstein} and partially observable linear systems~\cite{hakobyan2024wasserstein}, often preserving structural properties such as linearity of optimal controllers~\cite{taskesen2023distributionally}. In reinforcement learning, distributional robust approaches similarly aim to ensure robustness to model inaccuracies, with recent methods addressing uncertain dynamics and reward distributions, particularly in offline scenarios~\cite{moos2022robust,shi2024distributionally}. Across these applications, DRO enhances reliability by explicitly optimizing against worst-case distributions, improving performance in uncertain and safety-critical environments.


